Model-Based Reinforcement Learning with Adversarial Training for Online Recommendation

Reinforcement learning is well suited for optimizing policies of recommender systems. Current solutions mostly focus on model-free approaches, which require frequent interactions with the real environment, and thus are expensive in model learning. Offline evaluation methods, such as importance sampling, can alleviate such limitations, but usually request a large amount of logged data and do not work well when the action space is large. In this work, we propose a model-based reinforcement learning solution which models user-agent interaction for offline policy learning via a generative adversarial network. To reduce bias in the learned model and policy, we use a discriminator to evaluate the quality of generated data and scale the generated rewards. Our theoretical analysis and empirical evaluations demonstrate the effectiveness of our solution in learning policies from the offline and generated data.

==> prevmethod.tex <==
\section{Previous Method Part} 
\iffalse
\begin{algorithm}[t]
    \SetAlgoLined
    \KwIn{Offline data $\mathcal{B}^r$; an agnet model $A$; a user behavior model $U$; a discriminator $D$.}
    
    %\KwResult{$U_\theta$: user behavior model(not fixed), discriminator $D_\phi$, Roll-out policy $G_\beta$.}
    Initialize an empty simulated trajectories set $\mathcal{B}^f$.

    Initialize $U,A$ and $D$ with random parameters.

    Pre-train $U$ by minimizing Eqn. (\ref{ubm_loss}).

    Pre-train $A$ via policy gradient Eqn. (\ref{pg_estimator}) using $\mathcal{B}^r$ with reward function (\ref{reward_func}).

    Generate simulated trajectories using $A$ and $U$ for training $D$, and add to $\mathcal{B}^f$.

    Pre-train $D$ according to Eqn. (\ref{d_obj_func}) using $\mathcal{B}^r$ and $\mathcal{B}^f$.\\


    \For{$e\leftarrow 1$ \KwTo $epoch$}{
        \For{$\rm g-steps$}{
            Generate a simulated trajectory $\tau$ $\sim$ $A$ and $U$, and add to $\mathcal{B}^f$.

            Compute $q_{D}^{UA}(\tau_{1:t})$ at each step $t$ by Eqn. (\ref{rollout_reward}).
                
            Update U via policy gradient Eqn. (\ref{user_pg_estimator}) with $q_{D}^{UA}$ and A via policy gradient Eqn.~(\ref{pg_estimator}) with modified reward function (\ref{new_reward_func}).
            
            Update A using mini-batch sampled from $\mathcal{B}^r$ with reward function (\ref{reward_func}).
            
            %Update A via policy gradient Eqn. (\ref{pg_estimator}) with modified reward function (\ref{new_reward_func}).
        }
        \For{$\rm d-steps$}{
            Sample minibatch of $b_t$ trajectories from $\mathcal{B}^f$ and minibatch of $b_f$ trajectories from $\mathcal{B}^r$.
           
           Update D according to Eqn.(\ref{d_obj_func}) using sampled minibatch.
        }
    }
    \caption{InteractiveRecGAN}
\end{algorithm}
\fi
This section illustrates details of our reinforcement learning framework. Figure \ref{fig:model_overview} is the overview of our model, and section 4.1 shows the interactive model, and section 4.2 shows the adversarial training mechanism with the discriminator. The algorithm is shown in the supplementary material.
\subsection{Interactive model}

    %We now present our model-based deep reinforcement learning algorithm. We detail our agent model in \ref{agent_model}, our learned user behavior model in \ref{im1}, how to train the model in \ref{im2}, how to extract a policy with our learned model in \ref{im3}. and how to use reinforcement learning to further improve our learned model in \ref{im4}.

\subsubsection{Agent model learning} \label{agent_model}
     
    %For each user, we consider a sequence of user historical interactions with the recommnder, recording the actions taken by the system, i.e., recommended items, as well as user feedback, such as clicks and purchases. Given such a sequence, the recommender predicts the next action to take, i.e., items to recommend, so that user satisfaction metrics improve.
    
    The recommendation process can be formed as a typical reinforcement learning problem and solved by different families of methods. Here we translate this setup into an LSTM based agent model optimized by policy gradient approach, parameterized by $\theta_a$. At each step, the model would take as input the current click $c_t$ of the user and the historical hidden state $\textbf{h}^a_{t-1}$, output the updated state $\textbf{h}^a_{t}$ and next recommendation $R_t$ from a discrete item space $\mathcal{A}$ containing items available for recommendation according to a policy $\pi_{\vartheta_a}(R_t|\textbf{h}^a_t)$ parameterized by $\vartheta_a$, formally as
    \begin{align}
         &\textbf{h}^a_{t} = \mathbf{LSTM}(\textbf{h}^a_{t-1}, \bm{e}(c_t); \theta_a),\\
         &\pi_{\vartheta_a}(R_t|\textbf{h}^a_t)=\mathbf{softmax}(\textbf{W}_{\vartheta_a}\textbf{h}_{t}+\textbf{b}_{\vartheta_a}) 
    \end{align}
    
    where $\bm{e}(c)$ is the item embedding of $c$, so as to maximize the expected cumulative reward: $\textbf{max}_{\pi_{\vartheta_a}}\mathbb{E}_{\tau\sim\pi_{\vartheta_a}}[\sum_{t=0}^{|\tau|}r_t]$, where $r_t$ is the immediate reward at step $t$, $\tau$ is an interactive trajectory $({c}_1,{R}_1,{c}_2,\cdots)$. Furthermore, the gradient of the objective function $\mathbb{E}_{\tau\sim\pi_{\vartheta_a}}[\sum_{t=0}^{|\tau|}r_t]$ can be computed and estimated as follows:
     \begin{align}
        &\mathbb{E}_{\tau\sim\pi_{\vartheta_a}}[\big(\sum_{t=0}^{|\tau|}r_t\big)\nabla_{\vartheta_a} \textbf{log}\pi_{\vartheta_a}(\tau)]\approx \mathbb{E}_{\tau\sim\pi_{\vartheta_a}}[\big(\sum_{0}^{|\tau|}r^c_t\big)\nabla_{\vartheta_a} \textbf{log}\pi_{\vartheta_a}(\tau)], \label{pg_estimator}\\
        &r^c_t = \sum_{t'=t}^{|\tau|}\gamma^{t'-t}r_t,\label{cum_reward}
     \end{align}
      %And $c_1$ is sampled from an initial item distribution $\rho_0$. 
    %where $\gamma$ is the discount factor for future rewards to reduce variance in the gradient estimate  
    where $\gamma$ is the discount factor for future rewards and $r_t^c$ is the discounted cumulative reward. Although the estimator of the policy gradient is unbiased only in on-line reinforcement learning, where the policy gradient is computed on trajectories generated by the policy under consideration, we can still pre-train the agent model with the estimator from offline data.
    

\subsubsection{User behavior model learning} \label{im1}
    %In model-based reinforcement learning, an environment model is used to make prediction of user behavior given the recommendation by the agent. The model takes the current click $c_t$ and recommendation list $R_t$ and outputs an estimate of the next click at time $t+1$ and meanwhile predict the probability whether to purchase it. 
    
    We model the user as anthoer LSTM cell, parameterized by $\theta_u$. Formally, the model encodes the click history $C=c_1c_2\cdots c_t$ into a sequence of hidden states as follows:
    \begin{align}
    \textbf{h}^u_{t} = \mathbf{LSTM}(\textbf{h}^u_{t-1}, \bm{e}(c_t);\theta_u)    
    \end{align}
    
    where $\textbf{h}^u_{t}$ denotes the hidden state of the user behavior model at step $t$. And at each step, the will generate next click by choosing its favorite item from the distribution $\mathcal{P}(c_{t+1}|\textbf{h}^u_{t}, R_t)$ over all the recommended items, which is computed as follows:
    \begin{align}
            &\mathcal{P}(c_{t+1}|\textbf{h}^u_{t}, R_t) = \mathbf{softmax}(\mathcal{R}_t^u), \label{predict_click}\\
            &\mathcal{R}_t^u = e(R_t)^T(\textbf{W}_{\vartheta_u^c}\textbf{h}^u_{t}+\textbf{b}_{\vartheta_u^c})
    \end{align}
    where the relative value of each row in $\mathcal{R}_t^u$ means how the user likes the corresponding item in $R_t$. During interactive training, the item with maximum probability is set as the next click. Simultaneously the model needs to decides the probability $p_{t+1}(\textbf{h}_{t}, c_{t+1})$ whether to purchase the chosen item by another network, formally as,
    \begin{align}
        p_{t+1}(\textbf{h}^u_{t}, c_{t+1}) = \mathbf{sigmoid}(e(c_{t+1})^T(\textbf{W}_{\vartheta_u^p}\textbf{h}^u_{t}+\textbf{b}_{\vartheta_u^p}))  \label{predict_click}        
    \end{align}

    The total loss function $\Phi$ consists of click prediction error %$\Phi_c$
    and purchase prediction error %$\Phi_p$
    , which are computed as:
    \begin{align}
        %\Phi&=\Phi_c+\lambda_p\Phi_p,\label{ubm_loss}\\
        %\Phi_c&=\sum_{t}\big(\mathcal{P}(c_{t+1}=\tilde{c}_{t+1}|\textbf{h}^u_{t}, \tilde{R}_t)-1\big)^2,\\
        %\Phi_p&=\sum_{t}\big(p_{t+1}(\textbf{h}^u_{t}, \tilde{c}_{t+1})-\tilde{p}_{t+1}\big)^2,  
        \Phi&=\sum_{t}\big(\mathcal{P}(c_{t+1}=\tilde{c}_{t+1}|\textbf{h}^u_{t}, \tilde{R}_t)-1\big)^2+\lambda_p\sum_{t}\big(p_{t+1}(\textbf{h}^u_{t}, \tilde{c}_{t+1})-\tilde{p}_{t+1}\big)^2 \label{ubm_loss}
    \end{align}

    where $\tilde{c}_{t+1}$ is the real clicked item and $\tilde{p}_{t+1}$ is the real purchase probability (1 if $\tilde{c}_{t+1}$ was purchased otherwise 0), $\lambda$ is a scalar factor to balance two errors.
    
\subsubsection{Pre-Training} \label{im2}
    We collect interactive trajectories $\tilde\tau=(\tilde{c}_1,\tilde{R}_1,\tilde{p}_2,\cdots,\tilde{c}_{T-1},\tilde{R}_{T-1},\tilde{p}_T,\tilde{c}_T)$ from the offline dataset for pre-training both the agent model $A$ and the user behavior model $U$. Specially, the user behavior model should be trained to know when to finish the current interactive session with the recommender. Therefore we add a special terminal symbol $EOS$ to all $\tilde{R}_t$ and also add the symbol to end of each trajectory. To encourage the user to click and purchase as many items as possible, $r_t$ is computed as 
    \begin{equation}
        r_t(c_{t+1},p_{t+1})=\textbf{I}(c_{t+1}) + \lambda_r p_{t+1},\label{reward_func}
    \end{equation}
    where $\textbf{I}(c_{t+1})$ is 1 if $c_{t+1}$ is not $EOS$ otherwise 0 and $\lambda_r$ is another scale factor. In this way the agent model and user behavior model can be pre-trained according to Eqn.~(\ref{pg_estimator}) and Eqn.~(\ref{ubm_loss}) given ($\{c_t\},\{r_t\},\{R_t\}, \{p_t\}$).


\subsubsection{Model-Based Planning} \label{im3}
    
    To train the agent model $A$ using the learned user behavior model $U$, together with a pre-defined reward function (\ref{reward_func}), we formulate a model-based controller that is both computationally tractable and robust to inaccuracies in the learned user behavior model. In our experiment, we use two replay buffers, $\mathcal{B}^r$ for storing real trajectories from the offline dataset, $\mathcal{B}^f$ for simulated trajectories. Learning and planning are accomplished by the same policy gradient method as Eqn. (\ref{pg_estimator}), operating on real trajectories in $\mathcal{B}^r$ for learning and on simulated trajectories in $\mathcal{B}^f$ for planning. Thus, here we only describe the way that the simulated trajectories are generated.
    
    %In each interactive session, at the beginning we draw the first user click $c_1$ from an initial click distribution $\rho_0$. Thus $A$ can provide its recommendation to $U$ based on the current click, and then get the next click and immediate reward from $U$. The process keep going until $U$ returns the pre-defined terminal symbol $EOS$. $A$ can be updated by computing the cumulative reward and policy gradient as Eqn.~(\ref{pg_estimator}) and (\ref{cum_reward}). Note that $U$ would be fixed while model-based planning.

\subsection{Adversarial Training with Discriminator}
    The estimator $U$ of user behavior is usually biased due to the constraint of the hypothesis model. And theoretically, larger amounts of low-quality simulated trajectories that can't perfectly reflect real human behavior can have a negative impact on the recommendation policy learning. 
    
    To improve the effectiveness of planning, we incorporate a discriminator $D$ inspired by the generative adversarial network (GAN) into the planning process. The discriminator is trained to differentiate simulated trajectories from real user trajectories and then provide guidance for improving $U$ to reduce the bias between $U$ and the real user behavior from real offline dataset $\mathcal{B}^r$. However, most discriminative models can only perform classification well for an entire trajectory rather than the unfinished one. Therefore in order to provide a more detailed signal to evaluate immediate behavior of $U$, we adopt a discriminator predicting the probability that a trajectory is real only for a finished one, but meanwhile apply an N-time Monte-Carlo search with a roll-out policy to sample unknown last interaction steps for unfinished trajectories. In this way, for any simulated trajectory $\tau_{1:t}=(c_1,R_1,p_2,\cdots,p_{t},c_{t})$ from interaction between $U$ and $A$, the immediate discriminative signal $q^{UA}_D$ can be computed as
    
    \begin{equation}
    \label{rollout_reward}
    q^{UA}_D(\tau_{1:t}) =\left\{
    \begin{aligned}
    &\frac1N\sum_{n=1}^ND(\tau_{1:T}^n),\tau_{1:T}^n\in MC^{UA}(\tau_{1:t};EOS)~~&{\rm for}~c_t {\rm ~is~not~} EOS,\\
    &D(\tau_{1:t}) ~~&{\rm otherwise},
    \end{aligned}
    \right.
    \end{equation}

    where $N$ is the time of performing Monte Carlo search, $MC^{UA}(\tau;EOS)$ means keeping Monte Carlo search with roll-out policy same as interaction between $U$ and $A$, starting from $\tau$ and rolling out to $EOS$. Thus $U$ and $A$ can be dynamically updated via policy gradient to further improve the quality of simulated trajectories iteratively. The gradient of the objective function $\mathbb{E}_{\tau\sim\pi_{\vartheta_u}}[\sum_{t=0}^{|\tau|}q^{UA}_D(\tau_{1:t})]$ w.r.t. $U$'s parameter $\theta_u$ can be derived as follows:
    \begin{align}
        &\mathbb{E}_{\tau\sim\pi_{\vartheta_u}}[\big(\sum_{t=0}^{|\tau|}q^{UA}_D(\tau_{1:t})\big)\nabla_{\vartheta_u} \textbf{log}\pi_{\vartheta_u}(\tau)]\approx \mathbb{E}_{\tau\sim\pi_{\vartheta_u}}[\sum_{0}^{|\tau|}q^{UA}_D\nabla_{\vartheta_u} \textbf{log}\pi_{\vartheta_u}(\tau)]  \label{user_pg_estimator}
        %&q^c_t = \sum_{t'=t}^{|\tau|}\gamma^{t'-t}q^{UA}_D(\tau_{1:t}),\label{user_cum_reward}
    \end{align}
    
    At this stage, the agent $A$ can receive rewards from $U$ and $D$ meanwhile. The reward from the environment $U$ indicates the quality of the recommendation, while the reward from the discriminator $D$ indicates how much faith $A$ should have in the simulated trajectory in the update. Therefore, the reward function (\ref{reward_func})
    should be changed to:
    
    \begin{equation}
        r_t(c_{t+1},p_{t+1})=q_{D}^{UA}(\tau_{1:t})[\textbf{I}(c_{t+1}) + \lambda_r p_{t+1}] \label{new_reward_func}
    \end{equation}
    By using the modified reward function, $A$ can be updated via policy gradient Eqn.~(\ref{pg_estimator}) with less variance. Furthermore, once we have a set of more realistic trajectories, we shall train $D$ as follows:
    \begin{align}        \textbf{max}_{D}\mathbb{E}_{\tau\in \mathcal{B}^r}[\textbf{log} D(\tau)] + \mathbb{E}_{\tau\in\mathcal{B}^f}[\textbf{log} (1-D(\tau))] \label{d_obj_func}
    \end{align}
    

\subsubsection{Discriminator Model}
    Similarly, $D$ employs an LSTM parameterized by $\theta_d$ to encode a trajectory $\tau$ as a sequence of hidden states, and multi-layer perceptrons to output a probability indicating whether the trajectory looks like being generated by real users. We first represent the hidden state of $D$ as $\textbf{h}^d_{t}$ with LSTM:
    %\begin{align}
        %\textbf{h}^d_{t} = \mathbf{LSTM}(\textbf{h}^d_{t-1}, \bm{e}(c_t);\theta_d), \label{dis_lstm}
    %\end{align}
    Then the discriminative probability is computed as:
    \begin{align}
        &D(\tau) = \mathbf{sigmoid}\big[\frac{1}{|\tau|}\sum_{t=1}^{|\tau|}e(c^{{\rm max}}_{R_t})^Te(c_{t+1})\mathcal{W}_t^d\big], \label{dis_prob}\\
        &c^{{\rm max}}_{R_t}=\mathbf{argmax}_{c\in R_t}e({c})^T(\textbf{W}_{\vartheta_d^c}\textbf{h}^d_{t}+\textbf{b}_{\vartheta_d^c}),\\
        &\mathcal{W}_t^d=\textbf{W}_{\vartheta_d^p}p_{t+1}+\textbf{b}_{\vartheta_d^p},
    \end{align}
    where $c^{{\rm max}}_{R_t}$ represents the user's favorite item of the given $R_t$, and should be as close to $c_{t+1}$ as possible for real user. To ensure the gradient backpropagation, we use softmax with a temperature 0.1 to approximate the argmax function. Furthermore, $\mathcal{W}_t^d\in \mathbb{R}$ means the weight factor computed from $p_{t+1}$, which should be larger when $c_{t+1}$ is purchased. The optimization target of $D$ is formulated as Eqn.~(\ref{d_obj_func}).
    
\subsubsection{Joint Training}

    After the pre-training and model-based planning, $U$, $A$ and $D$ are Adversarially trained alternatively. As the user behavior model $U$ is updated according to Eqn.~(\ref{user_pg_estimator}) via getting discriminative signal from $D$ for u-steps , $D$ needs to be retrained periodically with real trajectories from the $\mathcal{B}^r$ and simulated ones from $\mathcal{B}^f$ according to Eqn.~(\ref{d_obj_func}) for d-steps to keep a good pace. Then the agent model $A$ can get the further upgrade by interacting with a less biased user behavior model. Moreover, the variance while training $A$ will be reduced because of the less bias between $\mathcal{B}^f$ and $\mathcal{B}^r$.

 

%\subsection{Towards online reinforcement learning}
